Understanding Deflation Process in Over-parametrized Tensor Decomposition

In this paper we study the training dynamics for gradient flow on over-parametrized tensor decomposition problems. Empirically, such training process often first fits larger components and then discovers smaller components, which is similar to a tensor deflation process that is commonly used in tensor decomposition algorithms. We prove that for orthogonally decomposable tensor, a slightly modified version of gradient flow would follow a tensor deflation process and recover all the tensor components. Our proof suggests that for orthogonal tensors, gradient flow dynamics works similarly as greedy low-rank learning in the matrix setting, which is a first step towards understanding the implicit regularization effect of over-parametrized models for low-rank tensors.

==> nonortho.tex <==
\section{Dynamics for Non-Orthogonal Tensors}

The proof in the orthogonal setting gives intuition to the dynamics in the non-orthgonal setting. Similar as before, we expect the direction of randomly initialized columns to evolve according to gradient flow while the residual does not change by much, and the column with the largest correlation with the residual will become much larger and eventually reduce the residual. However, unlike the orthogonal setting, in this case the columns that were already large will not stay where they are. This suggests a greedy-low-rank learning process as in Algorithm...

\rong{write the greedy-low rank algorithm}

The greedy-low-rank tensor decomposition algorithm is similar to the greedy-low-rank algorithm in \cite{} for analyzing implicit regularization for matrix problems. However, in the matrix case the column with the largest correlation is easy to compute, while it is in general NP-hard to find the best rank-1 approximation for a tensor and the algorithm will need to rely on random initializations and hope to find a component with good correlation. In the worst-case, the greedy-low-rank process may need a large number of columns to fit the original tensor. 

\rong{Maybe we can have a theorem for the worst case, saying that greedy-low-rank will reduce the residual by at least something in each iteration --- this should follow from a similar technique as our previous paper but much easier}

\begin{theorem}\label{thm:nonortho}
Suppose $\fn{T^*} =1$ and $\delta_0 = \poly(\epsilon/d).$ After $O(\frac{d^4 \log(d/\epsilon)}{\epsilon^6})$ epochs, we have 
$$\fn{T-T^*}\leq \epsilon.$$
\end{theorem}

The proof of Theorem~\ref{thm:nonortho} is in Appendix~\ref{sec:non_ortho_proof}.
However, in practice we observe that the greedy-low-rank algorithm is highly effective, and the dynamics of gradient flow with small initialization is very similar to the greedy-low-rank algorithm.

\rong{Describe experiment result}

==> nonortho_proof.tex <==
\section{Proof for Non-orthogonal setting}\label{sec:non_ortho_proof}
\begin{lemma}\label{lem:norm_bound}
Suppose $T = \sum_{w \in S} w^{\otimes 4}/\ns{w},$ we have 
$$\sum_{w\in S} \ns{w}\leq d\fn{T}.$$
\end{lemma}
\begin{proofof}{Lemma~\ref{lem:norm_bound}}
We can lower bound $\fns{T}$ as follows,
\begin{align*}
    \fns{T} = \fns{\sum_{w \in S} \frac{w^{\otimes 4}}{\ns{w}}}
    =& \sum_{i,j,k,l \in [d]} \pr{\sum_{w\in S}\frac{w_i w_j w_k w_l}{\ns{w}} }^2\\
    \geq& \sum_{i,j \in [d]} \pr{\sum_{w\in S}\frac{w_i^2 w_j^2}{\ns{w}} }^2\\
    =& \sum_{i,j \in [d]} \pr{\sum_{w\in S}w_i^2 \bw_j^2 }^2\\
    \geq& \frac{\pr{\sum_{w\in S}\sum_{i,j \in [d]} w_i^2 \bw_j^2 }^2}{d^2}
    = \frac{\pr{\sum_{w\in S}\sum_{i\in [d]} w_i^2  }^2}{d^2} = \frac{\pr{\sum_{w\in S}\ns{w}}^2}{d^2},
\end{align*}
where the last inequality follows from Cauchy-Schwarz inequality and the second last equality holds because $\sum_{j\in [d]} \bw_j^2 = 1.$
\end{proofof}

\begin{lemma}\label{lem:good_correlation}
Assume $\fn{T^*}=1.$
Suppose the residual is $T-T^*$ and the gradient is zero, we have  
$$\min_{u} (T-T^*)(\bu^{\otimes 4}) \leq -\frac{\fns{T-T^*}}{d}.$$
\end{lemma}
\begin{proofof}{Lemma~\ref{lem:good_correlation}}
Denote $T^* = \sum_{u \in S^*} u^{\otimes 4}/\ns{u}.$ According to Lemma~\ref{lem:norm_bound}, we have $\sum_{u\in S^*}\ns{u}\leq d.$ Suppose $T= \sum_{w\in S}w^{\otimes 4}/\ns{w}.$ We have 
\begin{align*}
    0 =& \frac{1}{2}\fns{ T-T^* - (\sum_{w\in S}w^{\otimes 4}/\ns{w} - \sum_{u \in S^*} u^{\otimes 4}/\ns{u})}\\
    =& \fns{T-T^*} -\sum_{w\in S}\ns{w}(T-T^*)(\bw^{\otimes 4}) + \sum_{v\in S}\ns{v}(T-T^*)(\bv^{\otimes 4}).
\end{align*}
Since the gradient equals zero, we know $\sum_{w\in S}\ns{w}(T-T^*)(\bw^{\otimes 4})=0.$ Therefore, we have 
$$\sum_{v\in S}\ns{v}(T-T^*)(\bv^{\otimes 4}) = -\fns{T-T^*},$$
which then implies $\min_{u} (T-T^*)(\bu^{\otimes 4}) \leq -\frac{\fns{T-T^*}}{d}.$
\end{proofof}


\begin{proofof}{Theorem~\ref{thm:nonortho}}
Since the function value only decreases, we have $\fn{T}=O(1),$ which then implies $\fns{W} = O(d).$ Suppose at the beginning of one epoch, we have $\fns{T-T^*}\geq \epsilon^2,$ according to Lemma~\ref{lem:good_correlation}, we know 
$$\min_{u} (T-T^*)(\bu^{\otimes 4}) \leq -\frac{\epsilon^2}{d}.$$
The running time would be $O(\frac{d}{\epsilon^2}\log(d/\epsilon)).$
Suppose the best correlation at the initialization is $\delta ,$ $\fns{W}$ is bounded by $M$ and the running time is $t$,
According to Lemma 9 in \cite{wang2020beyond},
$$\Delta f\geq \frac{\delta^2 }{M t} \geq \frac{1}{d}\cdot \frac{ \epsilon^2}{ d\log(d/\epsilon)} \cdot \pr{\frac{\epsilon^2}{d}}^2 = \frac{\epsilon^6}{d^4 \log(d/\epsilon)}.$$
Therefore, after $O(\frac{d^4 \log(d/\epsilon)}{\epsilon^6})$ epochs, we have 
$$\fn{T-T^*}\leq \epsilon. $$
\end{proofof}
